Resilient Sensor Fusion under Adverse Sensor Failures via Multi-Modal Expert Fusion

Modern autonomous driving perception systems utilize complementary multi-modal sensors, such as LiDAR and cameras. Although sensor fusion architectures enhance performance in challenging environments, they still suffer significant performance drops under severe sensor failures, such as LiDAR beam reduction, LiDAR drop, limited field of view, camera drop, and occlusion. This limitation stems from inter-modality dependencies in current sensor fusion frameworks. In this study, we introduce an efficient and robust LiDAR-camera 3D object detector, referred to as MoME, which can achieve robust performance through a mixture of experts approach. Our MoME fully decouples modality dependencies using three parallel expert decoders, which use camera features, LiDAR features, or a combination of both to decode object queries, respectively. We propose Multi-Expert Decoding (MED) framework, where each query is decoded selectively using one of three expert decoders. MoME utilizes an Adaptive Query Router (AQR) to select the most appropriate expert decoder for each query based on the quality of camera and LiDAR features. This ensures that each query is processed by the best-suited expert, resulting in robust performance across diverse sensor failure scenarios. We evaluated the performance of MoME on the nuScenes-R benchmark. Our MoME achieved state-of-the-art performance in extreme weather and sensor failure conditions, significantly outperforming the existing models across various sensor failure scenarios.

==> ex/supple/table_supple_5.tex <==
\begin{table*}[!h]
    \centering
    \tiny
    \setlength{\tabcolsep}{3pt}
    \renewcommand{\arraystretch}{1.15}
    \setlength{\arrayrulewidth}{0.3pt}
    % (a) Limited FOV table
    \begin{tabular}{@{}c|cc|cc|cc|cc|cc|cc@{\hspace{4pt}}}
       \toprule[0.1pt]
       \multirow{2}{*}[-2pt]{\tiny \hspace{2pt} Method} & \multicolumn{2}{c|}{Limited FOV} & \multicolumn{2}{c|}{Limited FOV} & \multicolumn{2}{c|}{Limited FOV} & \multicolumn{2}{c|}{Limited FOV} & \multicolumn{2}{c|}{Limited FOV} & \multicolumn{2}{c}{Limited FOV} \\ 
        
        \multicolumn{1}{c|}{} & \multicolumn{2}{c|}{\textit{[-180, 180]}} & \multicolumn{2}{c|}{\textit{[-150, 150]}} & \multicolumn{2}{c|}{\textit{[-120, 120]}} & \multicolumn{2}{c|}{\textit{[-90, 90]}} & \multicolumn{2}{c|}{\textit{[-60, 60]}} & \multicolumn{2}{c}{\textit{[-30, 30]}} \\
        \cline{2-13}
        & mAP & NDS & mAP & NDS & mAP & NDS & mAP & NDS & mAP & NDS & mAP & NDS \\ 
        \hline
        \hspace{2pt} CMT~\cite{cmt} & 70.3 & 72.9 & 65.4 & 69.8 & 53.8 & 62.2 & 49.0 & 58.4 & 43.9 & 54.0 & 35.0 & 46.1 \\
        \textbf{ \hspace{2pt} Immortal (ours)} & \textbf{71.2} & \textbf{73.6} & \textbf{67.8} & \textbf{71.2} & \textbf{56.2} & \textbf{63.4} & \textbf{54.2} & \textbf{61.2} & \textbf{50.6} & \textbf{58.3} & \textbf{44.0} & \textbf{53.0} \\ 
        \bottomrule[0.01pt]
    \end{tabular}
    \vspace{1em}
    
    % (b) Object Failure table
    \begin{tabular}{@{}c|cc|cc|cc|cc|cc|cc@{\hspace{4pt}}}
       \toprule[0.1pt]
       \multirow{2}{*}[-2pt]{\tiny \hspace{2pt} Method} & \multicolumn{2}{c|}{Object Failure} & \multicolumn{2}{c|}{Object Failure} & \multicolumn{2}{c|}{Object Failure} & \multicolumn{2}{c|}{Object Failure} & \multicolumn{2}{c|}{Object Failure} & \multicolumn{2}{c}{Object Failure} \\ 
        
        \multicolumn{1}{c|}{} & \multicolumn{2}{c|}{\textit{ratio=0.0}} & \multicolumn{2}{c|}{\textit{ratio=0.1}} & \multicolumn{2}{c|}{\textit{ratio=0.3}} & \multicolumn{2}{c|}{\textit{ratio=0.5}} & \multicolumn{2}{c|}{\textit{ratio=0.7}} & \multicolumn{2}{c}{\textit{ratio=0.9}} \\
        \cline{2-13}
        & mAP & NDS & mAP & NDS & mAP & NDS & mAP & NDS & mAP & NDS & mAP & NDS \\ 
        \hline
        \hspace{2pt} CMT~\cite{cmt} & 54.9 & 62.2 & 38.3 & 44.7 & 43.9 & 54.0 & 66.7 & 70.4 & 61.7 & 68.1 & 57.8 & 65.3 \\
        \textbf{ \hspace{2pt} Immortal (ours)} & \textbf{55.0} & \textbf{63.0} & \textbf{42.5} & \textbf{48.2} & \textbf{50.6} & \textbf{58.3} & \textbf{67.0} & \textbf{71.0} & \textbf{63.6} & \textbf{69.5} & \textbf{60.2} & \textbf{67.1} \\ 
        \bottomrule[0.01pt]
    \end{tabular}
    \vspace{1em}
    
    % (c) Beam Reduction table
    \begin{tabular}{@{}c|cc|cc|cc|cc|cc|cc@{\hspace{4pt}}}
       \toprule[0.1pt]
       \multirow{2}{*}[-2pt]{\tiny \hspace{2pt} Method} & \multicolumn{2}{c|}{Beam Reduction} & \multicolumn{2}{c|}{Beam Reduction} & \multicolumn{2}{c|}{Beam Reduction} & \multicolumn{2}{c|}{Beam Reduction} & \multicolumn{2}{c|}{Beam Reduction} & \multicolumn{2}{c}{Beam Reduction} \\ 
        
        \multicolumn{1}{c|}{} & \multicolumn{2}{c|}{\textit{1 beams}} & \multicolumn{2}{c|}{\textit{4 beams}} & \multicolumn{2}{c|}{\textit{8 beams}} & \multicolumn{2}{c|}{\textit{16 beams}} & \multicolumn{2}{c|}{\textit{24 beams}} & \multicolumn{2}{c}{\textit{32 beams}} \\
        \cline{2-13}
        & mAP & NDS & mAP & NDS & mAP & NDS & mAP & NDS & mAP & NDS & mAP & NDS \\ 
        \hline
        \hspace{2pt} CMT~\cite{cmt} & 54.9 & 62.2 & 38.3 & 44.7 & 43.9 & 54.0 & 61.7 & 68.1 & 63.2 & 69.4 & 64.5 & 70.2 \\
        \textbf{ \hspace{2pt} Immortal (ours)} & \textbf{55.0} & \textbf{63.0} & \textbf{42.5} & \textbf{48.2} & \textbf{50.6} & \textbf{58.3} & \textbf{63.6} & \textbf{69.5} & \textbf{65.4} & \textbf{70.8} & \textbf{66.8} & \textbf{71.8} \\ 
        \bottomrule[0.01pt]
    \end{tabular}
    \vspace{1em}
    
    % (d) View Drop table
    \begin{tabular}{@{}c|cc|cc|cc|cc|cc|cc@{\hspace{4pt}}}
       \toprule[0.1pt]
       \multirow{2}{*}[-2pt]{\tiny \hspace{2pt} Method} & \multicolumn{2}{c|}{View Drop} & \multicolumn{2}{c|}{View Drop} & \multicolumn{2}{c|}{View Drop} & \multicolumn{2}{c|}{View Drop} & \multicolumn{2}{c|}{View Drop} & \multicolumn{2}{c}{View Drop} \\ 
        
        \multicolumn{1}{c|}{} & \multicolumn{2}{c|}{\textit{1 drop}} & \multicolumn{2}{c|}{\textit{2 drops}} & \multicolumn{2}{c|}{\textit{3 drops}} & \multicolumn{2}{c|}{\textit{4 drops}} & \multicolumn{2}{c|}{\textit{5 drops}} & \multicolumn{2}{c}{\textit{6 drops}} \\
        \cline{2-13}
        & mAP & NDS & mAP & NDS & mAP & NDS & mAP & NDS & mAP & NDS & mAP & NDS \\ 
        \hline
        \hspace{2pt} CMT~\cite{cmt} & 54.9 & 62.2 & 38.3 & 44.7 & 43.9 & 54.0 & 66.7 & 70.4 & 61.7 & 68.1 & 58.2 & 66.5 \\
        \textbf{ \hspace{2pt} Immortal (ours)} & \textbf{55.0} & \textbf{63.0} & \textbf{42.5} & \textbf{48.2} & \textbf{50.6} & \textbf{58.3} & \textbf{67.0} & \textbf{71.0} & \textbf{63.6} & \textbf{69.5} & \textbf{61.7} & \textbf{68.1} \\ 
        \bottomrule[0.01pt]
    \end{tabular}

    \caption{Experimental comparisons on sensor corruptions with various degrees. (a) Limited FOV shows influence of reduced field of view, (b) Object Failure demonstrates robustness under varying object detection failures, (c) Beam Reduction evaluates performance with different LiDAR beam configurations, and (d) View Drop tests resilience against camera view losses. Our Immortal consistently outperforms CMT across all corruption settings.}
\label{table:sensor_corruptions}
\end{table*}

==> ex/table1.tex <==
\begin{table}[!h]
    \centering
    \footnotesize % 필요 시 폰트 크기 더 줄이기
    \label{tab1:results}
    \renewcommand{\arraystretch}{1.05}
    % tabularx 환경 사용, \columnwidth에 맞추기
    \begin{tabular}{@{\hspace{1em}}c|cc@{\hspace{1em}}}
        \hline
        Method  & mAP & NDS \\ 
        \hline
        %PETR \cite{petr} & C & 37.0 & 44.2 \\
        %BEVDet \cite{bevdet} & C & 39.3 & 47.2  \\
        %BEVFormer \cite{bevformer} & C & 41.6 & 51.7 \\
        %\hline
        %CenterPoint \cite{centerpoint} & L & 56.2 & 64.7 \\
        %TransFusion-L \cite{transfusion} & L & 65.1 & 70.1  \\
        %\hline
        % 3D-CVF \cite{3d-cvf}  & 42.2 & 49.8 \\
        MVP \cite{mvp} & 62.7 & 66.1 \\
        % UVTR \cite{uvtr}  & 65.4 & 70.2  \\
        TransFusion \cite{transfusion}  & 66.9 & 70.9 \\
        BEVFusion \cite{bevfusion_ADLAB}  & 67.9 & 71.0\\
        MetaBEV \cite{metabev}  & 68.0 & 71.5\\
        BEVFusion \cite{bevfusion_MIT}  & 68.5 & 71.4 \\
        MSMDFusion \cite{msmdfusion}  & 69.1 & 71.8 \\
        ObjectFusion \cite{objectfusion}  & 69.8 & 72.3  \\
        DeepInteraction \cite{deepinteraction}  & 69.9 & 72.6 \\
        GraphBEV \cite{graphbev}  & 70.1& 72.9 \\
        CMT \cite{cmt}  & 70.3 & 72.9 \\
        %FocalFormer3D \cite{focalformer3d}  & 70.5 & 73.1 \\
        UniTR \cite{unitr}  & 70.5 & 73.3\\
        SparseFusion \cite{sparsefusion}  & 71.0 & 73.1\\
        \hline
        \textbf{Immortal (Ours)}  & \textbf{71.2} & \textbf{73.6} \\ 
        \bottomrule
    \end{tabular}
     \caption{\textbf{Comparison with state-of-the-art methods on the nuScenes validation set.} Immortal achieves superior 3D performance even under clean sensor conditions.}
\label{tab1:results}
\end{table}



% \begin{table}[!h]
%     \centering
%     \footnotesize % 필요 시 폰트 크기 더 줄이기
%     \label{tab1:results}
%     \renewcommand{\arraystretch}{1.05}
%     % tabularx 환경 사용, \columnwidth에 맞추기
%     \begin{tabular}{@{\hspace{1em}}c|c|cc@{\hspace{1em}}}
%         \hline
%         Method & Modality & mAP & NDS \\ 
%         \hline
%         %PETR \cite{petr} & C & 37.0 & 44.2 \\
%         %BEVDet \cite{bevdet} & C & 39.3 & 47.2  \\
%         %BEVFormer \cite{bevformer} & C & 41.6 & 51.7 \\
%         %\hline
%         %CenterPoint \cite{centerpoint} & L & 56.2 & 64.7 \\
%         %TransFusion-L \cite{transfusion} & L & 65.1 & 70.1  \\
%         %\hline
%         % 3D-CVF \cite{3d-cvf}  & 42.2 & 49.8 \\
%         MVP \cite{mvp}  & 62.7 & 66.1 \\
%         % UVTR \cite{uvtr}  & 65.4 & 70.2  \\
%         TransFusion \cite{transfusion}  & 66.9 & 70.9 \\
%         BEVFusion \cite{bevfusion_ADLAB}  & 67.9 & 71.0\\
%         MetaBEV \cite{metabev}  & 68.0 & 71.5\\
%         BEVFusion \cite{bevfusion_MIT}  & 68.5 & 71.4 \\
%         MSMDFusion \cite{msmdfusion}  & 69.1 & 71.8 \\
%         ObjectFusion \cite{objectfusion}  & 69.8 & 72.3  \\
%         DeepInteraction \cite{deepinteraction}  & 69.9 & 72.6 \\
%         GraphBEV \cite{graphbev}  & 70.1& 72.9 \\
%         CMT \cite{cmt}  & 70.3 & 72.9 \\
%         %FocalFormer3D \cite{focalformer3d}  & 70.5 & 73.1 \\
%         UniTR \cite{unitr}  & 70.5 & 73.3\\
%         SparseFusion \cite{sparsefusion}  & 71.0 & 73.1\\
%         \hline
%         \textbf{Immortal (Ours)}  & \textbf{71.2} & \textbf{73.6} \\ 
%         \bottomrule
%     \end{tabular}
%      \caption{\textbf{Comparison with state-of-the-art methods on the nuScenes validation set.} `LC' denote camera, LiDAR, and LiDAR-Camera, respectively.}
% \label{tab1:results}
% \end{table}


==> ex/table5.tex <==
\begin{table}[t]
  \centering
  %\small % 글꼴 크기 줄이기

  \resizebox{0.35\textwidth}{!}{
  \begin{tabular}{@{}cccc@{}}
    \toprule
    \multicolumn{1}{c}{Method}& Latency (ms) & mAP & NDS \\
    \midrule
    Baseline \cite{cmt} & 270 & 70.3 & 72.9 \\
    M2E  & 310 & 33.4 & 51.8 \\
    Immortal (ours) & 274 (268+6) & \textbf{71.2} & \textbf{73.6} \\
    \bottomrule
  \end{tabular}
  }
  \caption{\textbf{Comparison of latency and performance.} Immortal demonstrates performance improvements over the baseline, with negligible additional latency from the AQR (+6 ms), achieving higher mAP and NDS.}
  \label{tab_5}
\end{table}


  
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     \multicolumn{1}{c}{Method}& FPS & mAP & NDS \\
%     \midrule
%     CMT \cite{cmt} & \textbf{3.7}& 70.3 & 72.9 \\
%     M2E  & 3.2 & 33.4 & 51.8 \\
%     Immortal & 3.5 & \textbf{71.2} & \textbf{73.6} \\
%     \bottomrule
%   \end{tabular}
%   \caption{\textbf{Comparison of performance and FPS.}}
%   \label{tab_5}
% \end{table}


==> sec/6_acknowledgement.tex <==
\section{Acknowledgement}

This work was partly supported by Institute of Information & communications Technology Planning & Evaluation (IITP) grant funded by the Korea government (MSIT)
[No.2021-0-01343-004, Artificial Intelligence Graduate School Program (Seoul National University)] and the National Research Foundation of Korea (NRF) grant funded by
the Korea government (MSIT) [No.2020R1A2C2012146].
